Sparsity Constrained Minimization via Mathematical Programming with Equilibrium Constraints

Sparsity constrained minimization captures a wide spectrum of applications in both machine learning and signal processing. This class of problems is difficult to solve since it is NP-hard and existing solutions are primarily based on Iterative Hard Thresholding (IHT). In this paper, we consider a class of continuous optimization techniques based on Mathematical Programs with Equilibrium Constraints (MPECs) to solve general sparsity constrained problems. Specifically, we reformulate the problem as an equivalent biconvex MPEC, which we can solve using an exact penalty method or an alternating direction method. We elaborate on the merits of both proposed methods and analyze their convergence properties. Finally, we demonstrate the effectiveness and versatility of our methods on several important problems, including feature selection, segmented regression, MRF optimization, trend filtering and impulse noise removal. Extensive experiments show that our MPEC-based methods outperform state-of-the-art techniques, especially those based on IHT.

==> mytable2.tex <==
%\begin{table*}[!t]
%\begin{center}
%\caption{$\ell_0$ norm optimization techniques.}\label{tab:l0opt}
%\begin{tabular}{|p{5.15cm}|p{8.15cm}|}
%  \hline
%  Method and Representative Reference & Description       \\
%  \hline
% \tabsize{ greedy descent methods \cite{mallat1993matching}}  & \tabsize{ only for smooth (typically quadratic) objective}   \\
%  \hline
%   \tabsize{ $\ell_1$ norm relaxation \cite{CandesT05}}  & \tabsize{$\|\bbb{x}\|_0 \approx \|\bbb{x}\|_1$}  \\
%  \hline
%   \tabsize{ $k$-support norm relaxation \cite{ArgyriouFS12}}  & \tabsize{$\|\bbb{x}\|_0 \approx \|\bbb{x}\|_{\text{k-sup}}$}  \\
%  \hline
%   \tabsize{ $k$-largest norm relaxation \cite{yu2011adversarial}}  & \tabsize{$\|\bbb{x}\|_0 \approx \|\bbb{x}\|_{\text{k-lar}}$}  \\
%  \hline
%  \tabsize{ QCQP convex relaxation \cite{Chan2007} } & \tabsize{$\|\bbb{x}\|_0\leq k \Rightarrow \|\bbb{x}\|_1 \leq \sqrt{k}\|\bbb{x}\|_2$}   \\
%  \hline
%   \tabsize{ SDP convex relaxation \cite{Chan2007} } & \tabsize{$\|\bbb{x}\|_0\leq k  \Rightarrow \bbb{X} = \bbb{xx}^T, ~\|\bbb{X}\|_1\leq k tr(\bbb{X})$} \\ %\|\bbb{x}\|_1^2 \leq k \|\bbb{x}\|_2^2
%  \hline
%   \tabsize{Schatten $\ell_p$ approximation \cite{GeJY11} } & \tabsize{$\|\bbb{x}\|_0 \approx \|\bbb{x}\|_p$}  \\
%  \hline
%   \tabsize{ re-weighted $\ell_1$ approximation \cite{candes2008enhancing}} & \tabsize{$\|\bbb{x}\|_0 \approx \la \textbf{1}, \ln(|\bbb{x}|+\epsilon)\ra $} \\
%  \hline
%   \tabsize{ $\ell_{\text{1-2}}$ DC approximation \cite{YinLHX15} } & \tabsize{$\|\bbb{x}\|_0 \approx \|\bbb{x}\|_1 - \|\bbb{x}\|_2 $} \\
%  \hline
%%  { truncated $\ell_1$ Section 4.5 in \cite{Dattorro2011} } & {$\|\bbb{x}\|_0 \approx \|\bbb{x}\|_1-\|\bbb{x}\|_{\text{top-k}}$} \\
%%  \hline
%  \tabsize{ $0\text{-}1$ mixed integer programming \cite{bienstock1996computational} }& \tabsize{$\{\|\bbb{x}\|_0:\|\bbb{x}\|_{\infty} \leq \lambda \} \Leftrightarrow \{\min_{\bbb{v}\in\{0,1\}}~\la \bbb{1},\bbb{v} \ra: |\bbb{x}|\leq \lambda \bbb{v}\}$} \\
%  \hline
% \tabsize{ iterative hard shreadholding \cite{LuZ13} } & \tabsize{$0.5\|\bbb{x}-\bbb{x}'\|_2^2,~s.t.~\|\bbb{x}\|_0\leq k$}  \\
%  \hline
%  \tabsize{ non-separable MPEC [This paper]} &\tabsize{$\|\bbb{x}\|_0 = \min_{\bbb{u}}~\|\bbb{u}\|_1, ~s.t. ~\|\bbb{x}\|_1 =  \la \bbb{x},\bbb{u} \ra,~-\bbb{1}\leq \bbb{u} \leq \bbb{1}$} \\
%  \hline
%  \tabsize{ separable MPEC \cite{YuanG15} [This paper]} & \tabsize{$\|\bbb{x}\|_0 = \min_{\bbb{v}}~\la \bbb{1}, \bbb{1}-\bbb{v}\ra, ~s.t.~|\bbb{x}|\odot \bbb{v}=\bbb{0},~\bbb{0}\leq \bbb{v}\leq \bbb{1}$} \\
%  \hline
%\end{tabular}
%\end{center}
%\vspace{-9pt}
%\end{table*}



 
\begin{table*}[!t]
%\small
\begin{center}
\centering
\caption{$\ell_0$ norm optimization techniques.}\label{tab:l0opt}
\scalebox{0.7}{\begin{tabular}{| P{4.9cm}| p{9.3cm}|} % %{| >{\centering\arraybackslash}m{1in} | >{\centering\arraybackslash}m{1in} |}
  \hline
    Method and Reference &  Description       \\
  \hline
 greedy descent methods & \multirow{2}{*}{ \tabsize{ only for smooth (typically quadratic) objective} }  \\
 \cite{mallat1993matching} &  \\
  \hline
$\ell_1$ norm relaxation & \multirow{2}{*}{ \tabsize{ $\|\bbb{x}\|_0 \approx \|\bbb{x}\|_1$ } }  \\
\cite{CandesT05}  &  \\
  \hline
$k$-support norm relaxation & \multirow{2}{*}{ \tabsize{ $\|\bbb{x}\|_0 \approx \|\bbb{x}\|_{\text{k-sup}} \triangleq \max_{\bbb{0}< \bbb{v}\leq \bbb{1}}~(\sum_{i}{\bbb{x}_i^2}/{\bbb{v}_i})^{1/2},~s.t.~\la \bbb{v} ,\bbb{1}\ra \leq k$ } }  \\
\cite{ArgyriouFS12}  &  \\
  \hline
$k$-largest norm relaxation & \multirow{2}{*}{ \tabsize{ $\|\bbb{x}\|_0 \approx \|\bbb{x}\|_{\text{k-lar}} \triangleq \max_{-\bbb{1}\leq \bbb{v}\leq \bbb{1}}~\la \bbb{v}, \bbb{x} \ra,~s.t.~\|\bbb{v}\|_{1}\leq k $ } }  \\
\cite{yu2011adversarial}  &  \\
  \hline
SOCP convex relaxation & \multirow{2}{*}{ \tabsize{ $\|\bbb{x}\|_0\leq k \Rightarrow \|\bbb{x}\|_1 \leq \sqrt{k}\|\bbb{x}\|_2$ } }  \\
\cite{Chan2007}  &  \\
  \hline
SDP convex relaxation & \multirow{2}{*}{ \tabsize{ $\|\bbb{x}\|_0\leq k  \Rightarrow \bbb{X} = \bbb{xx}^T, ~\|\bbb{X}\|_1\leq k tr(\bbb{X})$ } }  \\
\cite{Chan2007}  &  \\
  \hline
Schatten $\ell_p$ approximation & \multirow{2}{*}{ \tabsize{ $\|\bbb{x}\|_0 \approx \|\bbb{x}\|_p$ } }  \\
\cite{GeJY11}  &  \\
  \hline
re-weighted $\ell_1$ approximation & \multirow{2}{*}{ \tabsize{ $\|\bbb{x}\|_0 \approx \la \textbf{1}, \ln(|\bbb{x}|+\epsilon)\ra $ } }  \\
\cite{candes2008enhancing}  &  \\
  \hline
$\ell_{\text{1-2}}$ DC approximation  & \multirow{2}{*}{ \tabsize{ $\|\bbb{x}\|_0 \approx \|\bbb{x}\|_1 - \|\bbb{x}\|_2 $ } }  \\
\cite{YinLHX15}  &  \\
  \hline
 $0\text{-}1$ mixed integer programming  & \multirow{2}{*}{ \tabsize{ $\{\|\bbb{x}\|_0:\|\bbb{x}\|_{\infty} \leq \lambda \} \Leftrightarrow \{\min_{\bbb{v}\in\{0,1\}}~\la \bbb{1},\bbb{v} \ra: |\bbb{x}|\leq \lambda \bbb{v}\}$ } }  \\
\cite{bienstock1996computational}  &  \\
  \hline
iterative hard shreadholding & \multirow{2}{*}{ \tabsize{ $0.5\|\bbb{x}-\bbb{x}'\|_2^2,~s.t.~\|\bbb{x}\|_0\leq k$ } }  \\
\cite{LuZ13}  &  \\
  \hline
non-separable MPEC & \multirow{2}{*}{ \tabsize{ $\|\bbb{x}\|_0 = \min_{\bbb{u}}~\|\bbb{u}\|_1, ~s.t. ~\|\bbb{x}\|_1 =  \la \bbb{x},\bbb{u} \ra,~-\bbb{1}\leq \bbb{u} \leq \bbb{1}$ } }  \\
(\textcolor{red}{This paper})  &  \\
  \hline
separable MPEC \cite{YuanG15} (\textcolor{red}{This paper}) & \multirow{2}{*}{ \tabsize{ $\|\bbb{x}\|_0 = \min_{\bbb{v}}~\la \bbb{1}, \bbb{1}-\bbb{v}\ra, ~s.t.~|\bbb{x}|\odot \bbb{v}=\bbb{0},~\bbb{0}\leq \bbb{v}\leq \bbb{1}$ } }  \\
  \hline
\end{tabular}}
\end{center}
\end{table*}

